Lower Bounds for Possibly Divergent Probabilistic Programs

We present a new proof rule for verifying lower bounds on quantities of probabilistic programs. Our proof rule is not confined to almost-surely terminating programs -- as is the case for existing rules -- and can be used to establish non-trivial lower bounds on, e.g., termination probabilities and expected values, for possibly divergent probabilistic loops, e.g., the well-known three-dimensional random walk on a lattice.

==> macros.tex <==
% !TEX root = ./main.tex
%
\RequirePackage{todonotes}

% TODOS
%\setlength{\marginparwidth}{1.5cm}

\newcommand{\mccomment}[1]{\todo[color=blue!10,size=\small,fancyline,author=Mingshuai]{#1}\xspace}
\newcommand{\mccommentinline}[1]{\todo[inline,color=blue!10,author=Mingshuai]{#1}\xspace}
\newcommand{\atmc}{\colorbox{blue!10}{\textbf{@Mingshuai}}}

\newcommand{\sfcomment}[1]{\todo[color=green!10,size=\small,fancyline,author=Shenghua]{#1}\xspace}
\newcommand{\sfcommentinline}[1]{\todo[inline,color=green!10,author=Shenghua]{#1}\xspace}
\newcommand{\atsf}{\colorbox{green!10}{\textbf{@Shenghua}}}

\newcommand{\blkcomment}[1]{\todo[color=green!25,size=\small,fancyline,author=Benjamin]{#1}\xspace}
\newcommand{\blkcommentinline}[1]{\todo[inline,color=green!25,author=Benjamin]{#1}\xspace}
\newcommand{\atblk}{\colorbox{green!25}{\textbf{@Benjamin}}}

\newcommand{\hscomment}[1]{\todo[color=cyan!30,size=\small,fancyline,author=Han]{#1}\xspace}
\newcommand{\hscommentinline}[1]{\todo[inline,color=cyan!30,author=Han]{#1}\xspace}
\newcommand{\aths}{\colorbox{cyan!30}{\textbf{@Han}}}

\newcommand{\jpkcomment}[1]{\todo[color=orange!25,size=\small,fancyline,author=Joost-Pieter]{#1}\xspace}
\newcommand{\jpkcommentinline}[1]{\todo[inline,color=orange!25,author=Joost-Pieter]{#1}\xspace}
\newcommand{\atjpk}{\colorbox{orange!25}{\textbf{@Joost-Pieter}}}

\newcommand{\nzcomment}[1]{\todo[color=blue!25,size=\small,fancyline,author=Naijun]{#1}\xspace}
\newcommand{\nzcommentinline}[1]{\todo[inline,color=blue!25,author=Naijun]{#1}\xspace}
\newcommand{\atnz}{\colorbox{blue!25}{\textbf{@Naijun}}}

\newcommand{\rvcomment}[1]{\todo[color=red!10,size=\small,fancyline,author=Reviewer]{#1}\xspace}

\newcommand{\sfsymbol}[1]{\textsf{\upshape {#1}}}
\newcommand{\boldsfsymbol}[1]{\textbf{\textsf{\upshape {#1}}}}
\newcommand{\ttsymbol}[1]{\texttt{\upshape {#1}}}

%colors
\newcommand{\green}[1]{\textcolor{ForestGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\nblue}[1]{\textcolor{NavyBlue}{#1}}
\newcommand{\red}[1]{\textcolor{Red}{#1}}
\newcommand{\orange}[1]{\textcolor{RedOrange}{#1}}
\newcommand{\gray}[1]{\textcolor{Gray}{#1}}
\newcommand{\maroon}[1]{\textcolor{Maroon}{#1}}
\newcommand{\violet}[1]{\textcolor{Violet}{#1}}

%revision
\newcommand{\rev}[1]{\blue{#1}}
\newcommand{\add}[1]{\blue{#1}}
\newcommand\remove{\bgroup\markoverwith{\red{\rule[.4ex]{2pt}{1pt}}}\ULon}
\newcommand\removedisplay{\bgroup\markoverwith{\red{\rule[1ex]{2pt}{1pt}}}\ULon}
\everydisplay{\let\remove\removedisplay}
\newcommand{\change}[2]{\remove{#1}\add{#2}}

%marks
\newcommand{\cmark}{\textcolor{ForestGreen}{\ding{51}}}%
\newcommand{\xmark}{\textcolor{Maroon}{\ding{55}}}%
\newcommand{\namark}{\textcolor{Maroon}{\textbf{?}}}%

\newcommand{\Cmark}{\textcolor{ForestGreen}{\Large\ding{51}}}%
\newcommand{\Xmark}{\textcolor{Maroon}{\Large\ding{55}}}%
\newcommand{\NAmark}{\textcolor{Maroon}{\Large\textbf{?}}}%

\newcommand{\event}{\lozenge}

\newcommand{\toolname}[1]{\textsc{#1}} 

%for qedT mark compatible within displaymath
\def\triangleforqed{\hbox{$\lhd$}}
\makeatletter
\DeclareRobustCommand{\qedT}{%
	\ifmmode
	\eqno \def\@badmath{$$}%$$
	\let\eqno\relax \let\leqno\relax \let\veqno\relax
	\hbox{\triangleforqed}%
	\else
	\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
	\quad\hbox{\triangleforqed}%
	\fi
}
\makeatother

% weakest preexpectation
\newcommand{\wpsymbol}{\sfsymbol{wp}}
\newcommand{\boldwpsymbol}{\textbf{\sfsymbol{wp}}}
\renewcommand{\wp}[2]{\wpsymbol\llbracket #1\rrbracket\left(#2\right)}
\newcommand{\boldwp}[2]{\boldsymbol{\boldwpsymbol \left\llbracket {#1} \right\rrbracket \left( {#2} \right)}}
\newcommand{\extwp}[2]{\Ext{\wpsymbol}\llbracket#1\rrbracket\left(#2\right)}
\newcommand{\wpC}[1]{\wpsymbol\llbracket#1\rrbracket}

%fps
\newcommand{\fp}{\ensuremath{\textnormal{\sfsymbol{fp}}~}}
\newcommand{\lfp}{\ensuremath{\textnormal{\sfsymbol{lfp}}~}}
\newcommand{\gfp}{\ensuremath{\textnormal{\sfsymbol{gfp}}~}}

% functions

\newcommand{\measure}[2]{\prescript{#1}{}\!\mu_{#2}}
\newcommand{\probability}[1]{\prescript{#1}{}{\mathbb{P}}}
%\newcommand{\probability}[2]{\tensor*{^{#1}}{\mathbb{P}}{_{#2}}}
\newcommand{\expectv}[1]{\prescript{#1}{}{\EE}}
\newcommand{\poly}{\ensuremath{poly}\xspace}

\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\newcommand{\absd}[1]{\left\lvert#1\right\rvert}
\newcommand{\iverson}[1]{\left[ {#1} \right]}
\newcommand{\ket}[1]{\left|\, {#1} \right\rangle}
\newcommand{\bigiverson}[1]{\vphantom{\big(}\iverson{#1}\vphantom{\big)}}
\newcommand{\Min}[2]{\min\left\{\,{#1},\: {#2}\,\right\}}
\newcommand{\cemphMin}[2]{\cemph{\min}\left\{\,{#1},\: {#2}\,\right\}}
\newcommand{\Max}[2]{\max\left\{\,{#1},\: {#2}\,\right\}}
%\newcommand{\Exp}[2]{\sfsymbol{Exp}_{#1}\left( {#2} \right)}
\newcommand{\Exp}[2]{\int_\States \; {#2} \; d \,{#1} }
\newcommand{\ExpVals}[2]{\int_\Vals \; {#2} \; d \,{#1} }
\newcommand{\ERT}[2]{\sfsymbol{ERT}\left\llbracket #1 \right\rrbracket_{#2}}

%\newcommand{\Exp}[2]{\int_\States {#2} \: d {#1} }

\newcommand{\subst}[2]{\left[ {#1} \middle/ {#2}\right]}
\newcommand{\statesubst}[2]{\left[ {#1} \mapsto {#2}\right]}

%\newcommand{\charfun}[4]{\tensor*[^{#2}_{{#1}{#3}}]{\Phi}{_{{#4}}}}
\newcommand{\charfunaked}[1]{\Phi_{#1}}
\newcommand{\charfun}[4]{\tensor*[^{\smash{#1}}_{\smash{\langle #2, #3 \rangle}}]{\Phi}{_{{#4}}}}
\newcommand{\charfunn}[5]{\tensor*[^{#1}_{{\langle #2, #3 \rangle}}]{\Phi}{_{{#4}}^{{#5}}}}

\newcommand{\charfunnoguard}[2]{\tensor*[^{#1}]{\Phi}{_{{#2}}}}
\newcommand{\charfunnoguardn}[3]{\tensor*[^{#1}]{\Phi}{_{{#2}}^{{#3}}}}

\newcommand{\charwp}[3]{\charfun{\wpsymbol}{#1}{#2}{#3}}
\newcommand{\charwlp}[3]{\charfun{\wlpsymbol}{#1}{#2}{#3}}
\newcommand{\charawp}[3]{\charfun{\awpsymbol}{#1}{#2}{#3}}
\newcommand{\charawlp}[3]{\charfun{\awlpsymbol}{#1}{#2}{#3}}
\newcommand{\charert}[3]{\charfun{\ertsymbol}{#1}{#2}{#3}}
\newcommand{\charwpnoindex}[3]{{}^{\wpsymbol}\Phi_{#3}}
\newcommand{\charertnoindex}[3]{{}^{\ertsymbol}\Phi_{#3}}

\newcommand{\charwpn}[4]{\charfunn{\wpsymbol}{#1}{#2}{#3}{#4}}
\newcommand{\charwlpn}[4]{\charfunn{\wlpsymbol}{#1}{#2}{#3}{#4}}
\newcommand{\charawpn}[4]{\charfunn{\awpsymbol}{#1}{#2}{#3}{#4}}
\newcommand{\charawlpn}[4]{\charfunn{\awlpsymbol}{#1}{#2}{#3}{#4}}
\newcommand{\charertn}[4]{\charfunn{\ertsymbol}{#1}{#2}{#3}{#4}}
\newcommand{\charwpnnoindex}[4]{{}^{\wpsymbol}\Phi^{#4}_{#3}}
\newcommand{\charertnnoindex}[4]{{}^{\ertsymbol}\Phi^{#4}_{#3}}

\renewcommand{\eval}[1]{\ensuremath{\llbracket {#1} \rrbracket}}
\newcommand{\probof}[2]{\ensuremath{\llbracket {#1} \colon {#2} \rrbracket}}
\newcommand{\pot}[1]{\mathcal{P}\left({#1}\right)}

\newcommand{\sem}[3]{\left\llbracket #1 \right\rrbracket_{#2}^{#3}}

% program variables and states
\newcommand{\vars}{\mathtt{Vars}}
\newcommand{\pstate}{\ensuremath{\sigma}\xspace}
\newcommand{\States}{\mathit{\Sigma}}
\newcommand{\sink}{{\uparrow}}
\newcommand{\trace}{\ensuremath{s}\xspace}
\newcommand{\prefix}{\ensuremath{\pi}\xspace}
\newcommand{\cylinder}{\ensuremath{cyl}\xspace}

% Reals, Rationals...
\newcommand{\Nats}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\NatsInf}{\mathbb{N}^\infty\xspace}
\newcommand{\PosNats}{\ensuremath{\mathbb{N}_{>0}}\xspace}
\newcommand{\Ints}{\ensuremath{\mathbb{Z}}\xspace}
\newcommand{\Rats}{\ensuremath{\mathbb{Q}}\xspace}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\StrictPosReals}{\mathbb{R}_{> 0}}
\newcommand{\PosReals}{\mathbb{R}_{\geq 0}}
\newcommand{\PosRats}{\mathbb{Q}_{\geq 0}}
\newcommand{\PosRealsInf}{\mathbb{R}_{\geq 0}^\infty}

\newcommand{\RR}{\Reals}
\newcommand{\NN}{\Nats}

\newcommand{\EE}{\mathit{E}}
\newcommand{\FF}{\mathbb{E}}
\newcommand{\Expectations}{\FF}
\renewcommand{\SS}{\mathbb{S}}
\newcommand{\PP}{\mathbb{P}}

\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\newcommand{\primed}[1]{\ensuremath{{#1}^{\prime}}}

% Program Languages
\newcommand{\codify}[1]{\textup{\texttt{#1}}}
\newcommand{\pgcl}{\codify{pGCL}\xspace}
\newcommand{\gcl}{\codify{GCL}\xspace}

% Typesetting Program
% \newcommand{\IFSYMBOL}{\ensuremath{\textnormal{\texttt{if}}}}
% \newcommand{\IF}[1]{\ensuremath{\IFSYMBOL\,\left(\, {#1} \,\right)\,\{}}
% \newcommand{\ELSESYMBOL}{\ensuremath{\textnormal{\texttt{else}}}}
% \newcommand{\ELSE}{\ensuremath{\}\,\ELSESYMBOL\,\{}}
% \newcommand{\ITE}[3]{\ensuremath{\IFSYMBOL\,\left(\, {#1} \,\right)\,\left\{\, {#2} \,\right\}\,\ELSESYMBOL\,\left\{\, {#3} \,\right\}}}
 \newcommand{\TRUE}{\ensuremath{\textnormal{\texttt{true}}}}
 \newcommand{\FALSE}{\ensuremath{\textnormal{\texttt{false}}}}
% 
% \newcommand{\WHILESYMBOL}{\ensuremath{\textnormal{\texttt{while}}}}
% \newcommand{\WHILE}[1]{\ensuremath{\WHILESYMBOL \left(\, {#1} \,\right)\left\{\right.}}
% 
% \newcommand{\WHILEDO}[2]{\ensuremath{\WHILESYMBOL \left(\, {#1} \,\right)\left\{\, {#2} \,\right\}}}

%\newcommand{\define}{\ \hspace{0pt}\widehat{=}\hspace{0pt}\ }


%%%%    PGCL PROGRAMS    %%%%
\newcommand{\SKIP}{\ttsymbol{skip}}
%\newcommand{\DIVERGE}{\ttsymbol{diverge}}
\newcommand{\EMPTY}{\ensuremath{\textnormal{\texttt{empty}}}}
\newcommand{\HALT}{\ensuremath{\textnormal{\texttt{halt}}}}
\newcommand{\ABORT}{\ensuremath{\textnormal{\texttt{abort}}}}
\newcommand{\DIVERGE}{\ensuremath{\textnormal{\texttt{diverge}}}}

\newcommand{\OBSERVE}[1]{\ensuremath{\textnormal{\texttt{observe}} ~ {#1}}}
\newcommand{\ASSUME}[1]{\ensuremath{\textnormal{\texttt{assume}} ~ {#1}}}
\newcommand{\ASSERT}[1]{\ensuremath{\textnormal{\texttt{assert}} ~ {#1}}}
%\newcommand{\CALL}[1]{\ensuremath{\textnormal{\texttt{call}} ~ {#1}}}

\newcommand{\AssignSymbol}{\mathrel{\textnormal{$\mathtt{\coloneqq}$}}}
\newcommand{\ASSIGN}[2]{\ensuremath{#1 \AssignSymbol #2}}
\newcommand{\UNIFORM}[2]{\ensuremath{\mathtt{uniform}\left(#1,#2\right)}}
\newcommand{\ASSIGNUNIFORM}[3]{\ensuremath{#1 \AssignSymbol \UNIFORM{#2}{#3}}}
\newcommand{\PASSIGNUNIFORM}[3]{\ensuremath{\PASSIGN{#1}{\UNIFORM{#2}{#3}}}}
\newcommand{\ALLOC}[2]{\ensuremath{{#1} \AssignSymbol \mathtt{new}\left( #2 \right)}}

\newcommand{\AVAILLOC}[1]{\PosNats}
%\newcommand{\AVAILLOC}[1]{\ensuremath{\mathrm{loc}(#1)}}

%\newcommand{\dereference}[1]{\overline{#1}}
%\newcommand{\dereference}[1]{{}^*\!{#1}}

\newcommand{\dereference}[1]{\texttt{<}\,#1\,\texttt{>}}
%\newcommand{\dereference}[1]{\angl{\,#1\,}}

\newcommand{\HASSIGN}[2]{\ensuremath{\dereference{#1} \AssignSymbol #2}}
\newcommand{\ASSIGNH}[2]{\ensuremath{#1 \AssignSymbol \dereference{#2}}}
\newcommand{\FREE}[1]{\ensuremath{\mathtt{free}(#1)}}

\newcommand{\AppAssignSymbol}{\mathrel{\textnormal{\texttt{:}}\hspace{-.1em}{\approx}}}
\newcommand{\PASSIGN}[2]{\ensuremath{#1 \AppAssignSymbol\hspace{.1em} #2}}

\newcommand{\SEMI}{\ensuremath{\,;\,}}
%\newcommand{\SEMI}{\ensuremath{\,\fatsemi\,}}
%\newcommand{\COMPOSE}[2]{\ensuremath{{#1}{\,\fatsemi}~ {#2}}}
%\newcommand{\COMPOSE}[2]{\ensuremath{{#1}{\,;}~ {#2}}}
%\newcommand{\COMPOSE}[2]{\ensuremath{{#1}{\fatsemi} \: {#2}}}
\newcommand{\COMPOSE}[2]{\ensuremath{{#1}{\,\fatsemi}~ {#2}}}
\newcommand{\PCHOICE}[3]{\ensuremath{\left\{\, {#1} \,\right\}\mathrel{\left[\,#2\,\right]}\left\{\, {#3} \,\right\}}}
\newcommand{\NDCHOICE}[2]{\ensuremath{\left\{\, {#1} \,\right\}\mathrel{\Box}\left\{\, {#2} \,\right\}}}
\newcommand{\NDBRACK}{\ensuremath{\left.\right\}\mathrel{\Box}\left\{\right.}}


\newcommand{\IFSYMBOL}{\ensuremath{\textnormal{\texttt{if}}}}
\newcommand{\IF}[1]{\ensuremath{\IFSYMBOL\,\left(\, {#1} \,\right)\,\{}}
\newcommand{\ELSESYMBOL}{\ensuremath{\textnormal{\texttt{else}}}}
\newcommand{\ELSE}{\ensuremath{\}\,\ELSESYMBOL\,\{}}
\newcommand{\ITE}[3]{\ensuremath{\IFSYMBOL\,\left(\, {#1} \,\right)\,\left\{\, {#2} \,\right\}\,\ELSESYMBOL\,\left\{\, {#3} \,\right\}}}

\newcommand{\WHILESYMBOL}{\ensuremath{\textnormal{\texttt{while}}}}
\newcommand{\WHILE}[1]{\ensuremath{\WHILESYMBOL \left(\, {#1} \,\right)\left\{\right.}}

\newcommand{\WHILEDO}[2]{\ensuremath{\WHILESYMBOL \left(\, {#1} \,\right)\left\{\, {#2} \,\right\}}}

\newcommand{\TICKSYMBOL}{\ensuremath{\textnormal{\texttt{tick}}}}
\newcommand{\TICK}[1]{\ensuremath{\textnormal{\texttt{tick}} \left( #1 \right)}}


%%%%    Constants    %%%%%%%
\newcommand{\bb}{\ensuremath{\varphi}\xspace}
\newcommand{\cc}{\ensuremath{C}} % programs
\newcommand{\cloop}{\cc_{\textnormal{loop}}} % loop 
\newcommand{\pcloop}{\cc'_{\textnormal{loop}}} % loop 
\newcommand{\tcloop}{\cc^{\sink}_{\textnormal{loop}}} % loop 
\newcommand{\cgeo}{\cc_{\textnormal{geo}}} % loop 
\newcommand{\cloopp}{\cc^{\prime}_{\textnormal{loop}}} % loop prime
\newcommand{\fsub}[1]{\ensuremath{f_{\,#1}}\xspace}
\newcommand{\cbody}{\cc} % loop body 
\newcommand{\guard}{\bb} % conditial guard
\newcommand{\inv}{\ensuremath{\psi}\xspace}
\newcommand{\ee}{\ensuremath{e}} % expressions
\newcommand{\eeinfty}{\ensuremath{\tilde{e}}} % expressions or infty
\newcommand{\ea}{\ensuremath{a}} % expressions
\newcommand{\eainfty}{\ensuremath{\tilde{a}}} % expressions or infty
\newcommand{\eo}{\ensuremath{d}} % expressions
\newcommand{\eoinfty}{\ensuremath{\tilde{d}}} % expressions or infty

%%%%    Standards    %%%%

\newcommand{\mydot}{\text{{\Large\textbf{.}}~}}
\DeclareMathOperator{\dif}{\,d\!}
\newcommand{\TAG}[1]{{\tag*{\small{[{#1}]}}}}

%%%%    Shortcuts    %%%%

\newcommand{\tiff}{\textnormal{iff}\quad}
\newcommand{\qiff}{\ \quad\textnormal{iff}\quad\ }
\newcommand{\qqiff}{\qquad\textnormal{iff}\qquad}
\newcommand{\lqiff}{\textnormal{iff}\quad}
\newcommand{\lqqiff}{\textnormal{iff}\qquad}

\newcommand{\aand}{\ \ \textnormal{and}\ \ }
\newcommand{\qand}{\ \quad\textnormal{and}\quad\ }
\newcommand{\qqand}{\qquad\textnormal{and}\qquad}

\newcommand{\oor}{\ \ \textnormal{or}\ \ }
\newcommand{\qor}{\ \quad\textnormal{or}\quad\ }
\newcommand{\qqor}{\qquad\textnormal{or}\qquad}

\newcommand{\wwith}{\ \ \textnormal{with}\ \ }
\newcommand{\qwith}{\ \quad\textnormal{with}\quad\ }
\newcommand{\qqwith}{\qquad\textnormal{with}\qquad}

\newcommand{\qimplies}{\ \quad\textnormal{implies}\quad\ }
\newcommand{\qqimplies}{\qquad\textnormal{implies}\qquad}
\newcommand{\lqimplies}{\textnormal{implies}\quad}
\newcommand{\lqqimplies}{\textnormal{implies}\qquad}

\newcommand{\pprec}{\mathrel{{\prec}\hspace{-.5ex}{\prec}}}
\newcommand{\ppprec}{~{}\pprec{}~}
\newcommand{\npprec}{\centernot\pprec}


\newcommand{\ppreceq}{~{}\preceq{}~}
\newcommand{\ssucceq}{~{}\succeq{}~}
\newcommand{\defeq}{{}\triangleq{}}
\newcommand{\ddefeq}{\ {}\defeq{}\ }
\newcommand{\eeq}{~{}={}~}
\renewcommand{\mmapsto}{~{}\mapsto{}~}
\newcommand{\eequiv}{~{}\equiv{}~}
\newcommand{\pplus}{~{}+{}~}
\newcommand{\ccdot}{~{}\cdot{}~}
\newcommand{\llongrightarrow}{~{}\longrightarrow{}~}
\newcommand{\qlongrightarrow}{\quad{}\longrightarrow{}\quad}
\newcommand{\qqlongrightarrow}{\qquad{}\longrightarrow{}\qquad}
\newcommand{\mmid}{~{}\mid{}~}
\newcommand{\qmid}{\quad{}|{}\quad}
\newcommand{\tto}{~{}\to{}~}
\newcommand{\uuplus}{\,{}\uplus{}\,}
\newcommand{\nneq}{~{}\neq{}~}
\newcommand{\qeq}{\quad{}={}\quad}
\newcommand{\qqeq}{\qquad{}={}\qquad}
\newcommand{\lleq}{~{}\leq{}~}
\newcommand{\LL}{~{}<{}~}
\newcommand{\GG}{~{}>{}~}
\newcommand{\ggeq}{~{}\geq{}~}
\newcommand{\ssqsubseteq}{~{}\sqsubseteq{}~}
\newcommand{\iimplies}{~{}\implies{}~}
\newcommand{\mmodels}{~{}\models{}~}
\newcommand{\nnotmodels}{~{}\not\models{}~}
\newcommand{\iin}{~{}\in{}~}
\newcommand{\nnotin}{~{}\not\in{}~}
\newcommand{\wwedge}{~{}\wedge{}~}
\newcommand{\vvee}{~{}\vee{}~}

\newcommand{\cwedge}{\,{}\wedge{}\,}

==> sections/sec_preliminary.tex <==
% !TEX root = ../main.tex
%
\section{Preliminaries on Measure Theory}\label{sec:preliminary}
%\mccomment{We may prefer to drop this section and scatter preliminaries in the main sections instead.}\noindent
This section presents necessary preliminaries in measure theory which form the basis of understanding probabilistic programs. We refer interested readers to~\cite[Sect.~1.2]{dahlqvist_silva_kozen_2020} for a more detailed introduction to measure theory geared toward probabilistic programming.

\paragraph*{Basic Notations.}
Let $\Ints$, $\Rats$, and $\Reals$ be the set of integer, rational, and real numbers, respectively. For a set $\mathbb{K}$ of numbers, we denote by $\mathbb{K}_{\geq 0}$ the restriction of $\mathbb{K}$ to its non-negative elements, e.g., $\Ints_{\geq 0}$ coincides with the set $\Nats$ of natural numbers; and by $\mathbb{K}^\infty$ the extension of $\mathbb{K}$ with infinity.
%
%\subsection{Measure Theory}
%\mccomment{I collected some basic concepts here. But do we really need them? Would it weaken our results substantially if we keep everything discrete (and simply remark the extension to continuous distributions)?}

\paragraph*{Measurable Spaces and Functions.}
A \emph{$\sigma$-algebra} $\mathcal{B}$ on a set $S$ is a collection of subsets of $S$ containing the empty set $\emptyset$ that is closed under complementation in $S$ and countable union. The \emph{Borel $\sigma$-algebra} on $\RR$ -- consisting of \emph{Borel sets} on $\RR$ --  is the smallest $\sigma$-algebra on $\RR$ that contains the intervals. A pair $(S, \mathcal{B})$, where $S$ is a set and $\mathcal{B}$ is a $\sigma$-algebra on $S$, is called a \emph{measurable space}. Given two measurable spaces $(S, \mathcal{B}_S)$ and $(T, \mathcal{B}_T)$, a function $f\colon S\to T$ is \emph{measurable} if the inverse image $f^{-1}(B) = \{x \in S \mid f(x) \in B\}$ of every measurable subset $B \in \mathcal{B}_T$ is a measurable subset of $S$.

\paragraph*{(Sub)probability Measures.}
A \emph{signed (finite) measure} on a measurable space $(S, \mathcal{B})$ is a countably additive map $\mu \colon \mathcal{B} \to \Reals$ such that $\mu(\emptyset) = 0$. Note that $\mu$ is \emph{countably additive} means that if $\mathcal{A}$ is a countable set of pairwise disjoint events, then $\mu(\cup\mathcal{A}) = \sum_{A \in \mathcal{A}}\mu(A)$. A signed measure on $(S, \mathcal{B})$ is called \emph{positive} if $\mu(B) \geq 0$ for all $B \in \mathcal{B}$. A positive measure on $(S, \mathcal{B})$ is termed a \emph{probability measure} if $\mu(S) = 1$ and a \emph{subprobability measure} if $\mu(S) \leq 1$. A measurable set $B$ such that $\mu(B) = 0$ is called a \emph{$\mu$-nullset}, or simply a \emph{nullset} when it is clear from the context. A property over $S$ is said to hold \emph{($\mu$-)almost-surely} %($\mu$-a.s.) 
if the set of points on which it does not hold is contained in a nullset.
%
%A measure $\mu$ on a measurable space $(S, \mathcal{B})$ is \emph{continuous} if $\mu(\{s\}) = 0$ for all singleton sets $\{s\} \in \mathcal{B}$. A measure on a measurable space $(S, \mathcal{B})$ is \emph{discrete} if it is a countable weighted sum of \emph{Dirac measures} $\delta_s$ with $s \in S$ and $\delta_s(B) = 1$ if $s \in B$, while $0$ otherwise.

\paragraph*{Probability Spaces and Random Variables.}
A probability space $(\Omega, \mathcal{F}, P)$ consists of a sample space $\Omega$, a $\sigma$-algebra $\mathcal{F}$ on $\Omega$, and a probability measure $P\colon \mathcal{F} \to [0, 1]$ on the measurable space $(\Omega, \mathcal{F})$. A \emph{random variable} $X$ defined on the probability space $(\Omega, \mathcal{F}, P)$ is an $\mathcal{F}$-measurable function $X\colon \Omega \to \RR$; its $\emph{expected value}$ (w.r.t.\ $P$) is denoted by $\EE[X]$. Every random variable $X$ induces a (sub)probability measure $\mu_X\colon \mathcal{B} \to [0,1]$ on $\RR$, defined as $\mu_X(B) \defeq P(X^{-1}(B))$ for Borel sets $B$ in the Borel $\sigma$-algebra $\mathcal{B}$ on $\RR$. $\mu_X$ is also called the \emph{distribution of $X$}. $\mu_X$ is \emph{continuous} on the measurable space $(\RR, \mathcal{B})$ if $\mu(\{s\}) = 0$ for all singleton sets $\{s\} \in \mathcal{B}$; $\mu_X$ is \emph{discrete} if it is a countable weighted sum of \emph{Dirac measures} $\delta_s$ with $s \in S$ and $\delta_s(B) = 1$ if $s \in B$, and $0$ otherwise.
%; its \emph{support set} is $\supp(\mu_X) \define \overline{\bigcup_{\mu_X(B) > 0} B}$.

\paragraph*{Stochastic Processes and Stopping Times.}
A (discrete-time) \emph{stochastic process} is a parametrized collection of random variables $\{X_n\}_{n \in \NN}$. We sometimes drop the brackets in $\{X_n\}$ when it is clear from the context.\rvcomment{"of sigma-algebras on sets in F": this is confusing, I would not say they're sigma algebras "on sets in F"; they're sigma algebras on Omega that are subsets of F.}
A collection $\{\mathcal{F}_n\}_{n \in \NN}$ of $\sigma$-algebras on sets in $\mathcal{F}$ is a \emph{filtration} if $\mathcal{F}_n \subseteq \mathcal{F}_{m}$ for all $m \geq n$. Intuitively, $\mathcal{F}_n$ carries the information known to an observer at step $n$. A random variable $\tau\colon \Omega \to \NN$ is called a \emph{stopping time} w.r.t.\ some filtration $\{\mathcal{F}_n\}_{n \in \NN}$ of $\mathcal{F}$ if $\{\tau \le n\} \in \mathcal{F}_n$ for all $n \in \NN$. Given a stochastic process $X_n$ and a stopping time $\tau$, the \emph{stopped process} $\{X^\tau_n\}_{n \in \NN}$ is defined by
\begin{align*}
	X^\tau_n \ddefeq
	\begin{cases}
		X_n &\text{if}~n \leq \tau~,\\
		X_{\tau} &\text{if}~n > \tau~,
	\end{cases}%
\end{align*}%
namely, a process that is forced to keep the same value after a prescribed (random) time $\tau$.
%
%
%We refer interested readers to~\cite[Sect.~1.2]{dahlqvist_silva_kozen_2020} for a more detailed introduction to measure theory oriented toward probabilistic programming.
